Establishing Knowledge Preference in Language Models

Language models are known to encode a great amount of factual knowledge through pretraining. However, such knowledge might be insufficient to cater to user requests, requiring the model to integrate external knowledge sources and adhere to user-provided specifications. When answering questions about ongoing events, the model should use recent news articles to update its response; when asked to provide recommendations, the model should prioritize user specifications over retrieved product reviews; when some facts are edited in the model, the updated facts should override all prior knowledge learned by the model even if they are conflicting. In all of the cases above, the model faces a decision between its own parametric knowledge, (retrieved) contextual knowledge, and user instruction knowledge. In this paper, we (1) unify such settings into the problem of knowledge preference and define a three-level preference hierarchy over these knowledge sources; (2) compile a collection of existing datasets IfQA, MQuAKE, and MRQA covering a combination of settings (with/without user specifications, with/without context documents) to systematically evaluate how well models obey the intended knowledge preference; and (3) propose a dataset synthesis method that composes diverse question-answer pairs with user assumptions and related context to directly fine-tune LMs for instilling the hierarchy of knowledge. We demonstrate that a 7B model, fine-tuned on only a few thousand examples automatically generated by our proposed method, effectively achieves superior performance (more than 18% improvement across all evaluation benchmarks) in adhering to the desired knowledge preference hierarchy.

==> Contents/tables/tab_conflictQA.tex <==
\begin{table*}[!t]
    \small 
    \centering
    % \renewcommand\tabcolsep{3pt} % column space
    % \setlength{\tabcolsep}{12pt}
    \scalebox{1}{
    \begin{tabular}{lccc}
        \toprule 
        \multirow{1}{*}{Model} & \multirow{1}{*}{w/ Explicit Prompt} & Acc. on StrategyQA & Acc. on PopQA  \\ 
        \midrule
        \multirow{2}{*}{Mistral-v0.3-7B w/ Alpaca} & \okmark & 71.39 & 78.53 \\
                                                   & \ngmark & 72.46 & 78.38  \\
        \multirow{2}{*}{Mistral-v0.3-7B w/ \Ours}  & \okmark & 77.54 & 80.90 \\
                                                   & \ngmark & 79.09 & 81.52 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Evaluation results (\%) on ConflictQA given the document either aligned to the memory answer or to the counter-answer. Accuracy is reported. Following the original paper's setup, we formulate the question answering as a multiple choice problem with three randomly shuffled options: \texttt{Memory answer}, \texttt{Counter-answer}, and \texttt{Uncertain}. Here \texttt{w/ Explicit Prompt} refers to whether the explicit prompting strategy of Assumption-in-Question is applied or not. }
    \label{tab:eval_conflictQA_w_param_counter_docs}
\end{table*}
